FIESTA: Fisher Information-based Efficient Selective Test-time Adaptation

Robust facial expression recognition in unconstrained, "in-the-wild" environments remains challenging due to significant domain shifts between training and testing distributions. Test-time adaptation (TTA) offers a promising solution by adapting pre-trained models during inference without requiring labeled test data. However, existing TTA approaches typically rely on manually selecting which parameters to update, potentially leading to suboptimal adaptation and high computational costs. This paper introduces a novel Fisher-driven selective adaptation framework that dynamically identifies and updates only the most critical model parameters based on their importance as quantified by Fisher information. By integrating this principled parameter selection approach with temporal consistency constraints, our method enables efficient and effective adaptation specifically tailored for video-based facial expression recognition. Experiments on the challenging AffWild2 benchmark demonstrate that our approach significantly outperforms existing TTA methods, achieving a 7.7% improvement in F1 score over the base model while adapting only 22,000 parameters-more than 20 times fewer than comparable methods. Our ablation studies further reveal that parameter importance can be effectively estimated from minimal data, with sampling just 1-3 frames sufficient for substantial performance gains. The proposed approach not only enhances recognition accuracy but also dramatically reduces computational overhead, making test-time adaptation more practical for real-world affective computing applications.

==> sec/Y_topology.tex <==
\section{Topological Characterization of Adaptability Potential}

Although test-time adaptation techniques based on temporal smoothness assumptions have shown promise in stabilizing predictions and improving performance in unconstrained video, our empirical findings indicate that these benefits are inconsistent. Models may respond unpredictably to adaptation, and the absence of a principled mechanism for estimating whether adaptation will help or hinder performance presents a significant limitation. This is particularly true in domains such as facial expression understanding, where variation in data quality, facial morphology, and recording conditions is substantial. In such cases, blindly applying adaptation can lead to performance instability or reduced generalization.

To address this challenge, we developed a predictive framework that estimates a model’s adaptability prior to performing any adaptation. The goal was to create a lightweight and unsupervised mechanism that offers a reliable signal of the model’s compatibility with the adaptation objective, without modifying the model itself. We draw on recent advances in the topological analysis of neural networks and propose a diagnostic tool based on persistent homology.

\subsection{Motivation and Theoretical Foundation}

Persistent homology is a core technique in topological data analysis (TDA) that quantifies the shape of high-dimensional data by tracking the emergence and disappearance of topological features—such as connected components and loops—across varying scales. In the context of deep learning, this method enables the structural analysis of activation spaces, providing a rich and interpretable summary of how internal representations evolve in response to input data.

Our approach builds on the foundational work of \cite{guss2018characterizing}, who showed that persistent homology can be used to compare the complexity of neural representations across architectures. Further, \cite{corneanu2020computing} demonstrated that persistent topological summaries correlate with generalization and can be used to estimate test performance without labeled test data. These works collectively suggest that the internal structure of activations carries meaningful signals about a model’s generalization behavior. This insight forms the backbone of our method.

\subsection{Method Overview}

We propose a topological diagnostic pipeline that leverages persistent homology to assess whether a pretrained model is likely to benefit from test-time adaptation when applied to a new video sequence.

\begin{enumerate}
    \item \textbf{Activation Extraction:} The input sequence is passed through a fixed, pretrained model. We extract activations from intermediate layers—typically normalization or convolutional layers—which are known to encode meaningful, domain-general representations.

    \item \textbf{Graph Construction:} A similarity graph is constructed from the activation vectors, where nodes represent individual units and edges encode cosine similarity between their temporal activation profiles. This graph reflects how similarly neurons respond over time.

    \item \textbf{Filtration and Persistent Homology:} We apply a filtration on the graph by varying the similarity threshold and tracking the formation and dissolution of topological features using either Vietoris-Rips or flag complexes. This process yields persistence diagrams that describe the multiscale topological landscape of the activation graph.

    \item \textbf{Feature Vectorization:} The persistence diagrams resulting from the previous step capture multiscale topological features (birth-death pairs) across the activation graph. To transform these diagrams into fixed-length feature vectors amenable to machine learning, we compute a set of statistical descriptors. Specifically, for each diagram (typically computed for $\beta_0$ and $\beta_1$ homology), we calculate the following summary statistics:

    \begin{itemize}
        \item \textit{Persistence statistics:} We compute the mean, standard deviation, maximum, and total sum of lifetimes (i.e., death minus birth) across all points in the diagram. These capture the overall spread and intensity of topological features.
        \item \textit{Birth and death distributions:} We similarly summarize the distributions of birth times and death times using their respective means, standard deviations, and extrema. These offer insight into how quickly or persistently topological features form and dissolve during the filtration.
        \item \textit{Persistence entropy:} Following \cite{corneanu2020computing}, we compute the normalized entropy of the lifetime distribution, which reflects the diversity and informativeness of persistent features.
        \item \textit{Cardinality:} The total number of points in the diagram, optionally normalized by the number of nodes in the graph, provides a measure of topological complexity.
    \end{itemize}

All computed features are concatenated into a fixed-length vector, separately for $\beta_0$ and $\beta_1$, and then optionally aggregated across multiple layers if activations were extracted from more than one layer. These topological descriptors serve as a compact, interpretable representation of the model's internal dynamics over the input sequence and are used as input to the meta-classifier for adaptability prediction.

\item \textbf{Adaptability Estimation:} Finally, the topological descriptors are passed to a lightweight meta-classifier trained to estimate the expected benefit (or risk) of adaptation. This output serves as a decision gate for whether adaptation should be applied.
\end{enumerate}

\subsection{Application to Affwild2}

We evaluate our topological adaptation gating framework in the context of video-based facial expression recognition. Given the frame-wise nature of predictions and the substantial variability in recording conditions, subject demographics, and head motion, facial expression datasets are particularly susceptible to domain shift—making them a prime testbed for selective adaptation.

Our pipeline operates on video sequences independently. For each video, we extract intermediate activations from a pretrained facial expression recognition model and compute persistent homology-based descriptors as described above. These descriptors are then passed through a lightweight classifier to estimate the potential benefit or risk of applying test-time adaptation to the given sequence. This classification output serves as a gating mechanism: adaptation is only performed if the predicted benefit exceeds a learned threshold.

The meta-classifier itself is trained using the official training partition of the dataset. We construct a supervision signal by measuring the actual performance change induced by adaptation (e.g., change in mean squared error or classification accuracy) on training videos, labeling sequences as “adaptable” or “non-adaptable” accordingly. This allows the model to learn patterns in topological descriptors that correlate with successful adaptation.

All hyperparameters involved in the persistent homology computation and the meta-classifier are selected based on cross-validation within the training set. This ensures that the final model remains untouched during testing and that reported results are free from any test-time tuning bias.

At evaluation time, the pipeline is applied directly to each sequence in the test partition. Importantly, all components of the system—namely, the feature extraction layers, persistence-based summarization, and the classifier—remain fixed during this phase. The system autonomously determines whether adaptation should be applied for each test video, without any manual intervention or post hoc adjustments.

Empirical results confirm the utility of our method. When integrated into the overall facial expression recognition system, our selective adaptation mechanism consistently improves test-time performance over a naive adaptation baseline that applies adaptation indiscriminately to all sequences. Crucially, our method avoids the degradation observed when adapting on sequences for which the assumption of temporal coherence or feature smoothness is violated. This illustrates the practical value of incorporating topological reasoning into real-world video understanding tasks, particularly those involving human behavior and affect.

